Simple Length Rigidity for Hitchin Representations

We show that a Hitchin representation is determined by the spectral radii of the images of simple, non-separating closed curves. As a consequence, we classify isometries of the intersection function on Hitchin components of dimension 3 and on the self-dual Hitchin components in all dimensions. As an important tool in the proof, we establish a transversality result for positive quadruples of flags.

==> lengthtrace-resubmit_old.tex <==

%% !TEX root =HitchinSimple.tex
\section{Simple lengths and traces}
\label{lengthtrace}

We show that two Hitchin representations have the same simple non-separating length spectrum 
if and only if they have the same simple non-separating trace spectrum. Moreover, in either case all
eigenvalues of images of simple non-separating curves agree up to sign.

\begin{theorem}
\label{equivalence}
If $\rho,\sigma \in  {\mathcal H}_d(S)$, then
$|\tr(\rho(\alpha))|=| \tr(\sigma(\alpha))|$ for any \hbox{$\alpha\in\pi_1(S)$} represented by a simple non-separating curve
on $S$ if and only if  \hbox{$L_\alpha(\rho) = L_\alpha(\sigma)$}
for any $\alpha\in\pi_1(S)$ represented by a simple non-separating curve on $S$.
In either case, $\lambda_i(\rho(\alpha))=\lambda_i(\sigma(\alpha))$ for all $i$ and
any $\alpha\in\pi_1(S)$ represented by a simple non-separating curve on $S$.
\end{theorem}

Theorem \ref{equivalence} follows immediately from Lemma \ref{trace to length}, which shows that one can detect the length
of a curve from the traces of a related family of curves, and Lemma \ref{length to trace}, which obtains information
about traces and eigenvalues from information about length.

\begin{lemma}
\label{trace to length}
Suppose that $\alpha$ and $\beta$ are represented by  simple based loops on $S$ which intersect 
only at the basepoint  and have geometric intersection one.
If $\rho,\sigma \in  {\mathcal H}_d(S)$ and
$|\tr(\rho(\alpha^n\beta))|=|\tr(\sigma(\alpha^n\beta))|$ for all $n$, then $L_\alpha(\rho) = L_\alpha(\sigma)$.
Moreover, $\lambda_i(\rho(\alpha))=\lambda_i(\sigma(\alpha))$ for all $i$.
\end{lemma}

\begin{proof}
It suffices to prove our lemma for lifts of the restriction of $\rho$ and $\sigma$ to $\braket{\alpha,\beta}$ 
so that the all the eigenvalues of the images of $\alpha$ are positive.
We will abuse notation by calling these lifts $\rho$ and $\sigma$.

Since $\tr(\rho(\alpha^n\beta)) =\epsilon(n)\tr(\sigma(\alpha^n\beta))$ for all $n$, where $\epsilon(n) \in\{\pm 1\}$,
we may expand to see that
 $$\sum_i \lambda_i^n(\rho(\alpha))\tr(\p_i(\rho(\alpha))\rho(\beta)) = 
 \epsilon(n)\sum_i \lambda_i^n(\sigma(\alpha))\tr(\p_i(\sigma(\alpha))\sigma(\beta))$$
for all $n$.
Lemma \ref{tracenonzero-i0} implies that $\tr(\p_i(\rho(\alpha))\rho(\beta))$ and
$\tr(\p_i(\sigma(\alpha))\sigma(\beta))$ are non-zero for all $i$.
There exists an infinite subsequence $\{n_k\}$  of integers, so that $\epsilon(n_k) = \epsilon$
is constant.  Passing to limits as $n \rightarrow \infty$, and comparing the leading terms  in descending order,
we see that
$\lambda_i(\rho(\alpha))=\lambda_i(\sigma(\alpha))$ (and that
$\tr(\rho(\beta)\p_i(\rho(\alpha)))=\epsilon\tr(\sigma(\beta)\p_i(\sigma(\alpha)))$) for all $i$).
In particular, $L_\alpha(\rho)=L_\alpha(\sigma)$. 
\end{proof}

\begin{lemma}
\label{length to trace}
Suppose that $\gamma$ and $\delta$ are represented by  simple based loops on $S$ which intersect 
only at the basepoint  and have geometric intersection  one.
If $\rho,\sigma \in  {\mathcal H}_d(S)$ and
$L_{\beta}(\rho)=L_{\beta}(\sigma)$ whenever $\beta\in\braket{\gamma,\delta}$ is represented by
a simple non-separating based loop, then 
$|\tr(\rho(\alpha))|=|\tr(\sigma(\alpha))|$ and
$\lambda_i(\rho(\alpha))=\lambda_i(\sigma(\alpha))$ for all $i$ 
whenever $\alpha\in\braket{\gamma,\delta}$ is represented by
a simple non-separating based loop.
\end{lemma}

\begin{proof} 
If $\alpha\in\braket{\gamma,\delta}$ is represented by a simple, non-separating based loop, then there exists
$\beta\in\braket{\gamma,\delta}$  so that $\beta$ is represented by a simple based loop which intersects
$\alpha$ only at the basepoint and $\alpha$ and $\beta$ have geometric intersection  one, so $\alpha^n\beta$ is simple
and non-separating for all $n$.
It again suffices to prove our lemma for lifts of the restriction of $\rho$ and $\sigma$ to $\braket{\alpha,\beta}$ 
so that the all the eigenvalues of the images of $\alpha$ are positive.

Let $A = \rho(\alpha)$,  $B = \rho(\beta)$, $\hat A = \sigma(\alpha)$,  and $\hat B = \sigma(\beta)$.
Let $\lambda_i=\lambda_i(A)$ and $\hat\lambda_i=\lambda_i(\hat A)$.
Let $e_i=e_i(A)$ and $\hat e_i=e_i(\hat A)$ and let $(b^i_j)$ be the matrix of $B$ with respect to $\{e_i\}_{i=1}^d$
and $(\hat b^i_j)$ be the matrix of $\hat B$ with respect to $\{\hat e_i\}_{i=1}^d$.
Let $\Omega = e_1\w e_2\w \ldots \w e_d \neq 0$ be the volume form associated to the basis $\{e_1\}_{i=1}^d$ for
$\mathbb R^d$.


We begin by showing that $\lambda_2=\hat\lambda_2$.
Notice that $A$ and $A^nB$  are real-split and 2-proximal for all $n$.
We need the result of the following lemma to be
able to apply Lemma \ref{specradiusexpansion}.

\begin{lemma}
\label{nonzero coefficients}
Suppose that $\alpha$ and $\beta$ are represented by  simple based loops on $S$ which intersect 
only at the basepoint  and have geometric intersection  one. If $\rho\in\Hn$ and $B=(b_i^j)$ is a
matrix representing $\rho(\beta)$ in the basis $\{e_i(\rho(\alpha)\}$, then 
$b^1_1$, $b^1_2$, and $b^2_1$ are all non-zero.
\end{lemma}

\begin{proof}
Notice that $B(e_1)\w (e_{2}\w \ldots  \w e_d) = b^1_1\Omega$. So, if $b^1_1=0$, then 
$B(e_1)$, which is a non-trivial multiple of $e_1(\rho(\beta\alpha\beta^{-1}))$,
lies in the hyperplane spanned by
$\{e_2,\ldots,e_d\}=\{e_2(\rho(\alpha)),\ldots,e_d(\rho(\alpha)\}$,
which contradicts Corollary \ref{productnonzero} (and also hyperconvexity).
Notice that the fixed points of $\beta\alpha\beta^{-1}$ must lie in the same component of $\xi_\rho(S^1)-\{\alpha^+,\alpha^-\}$,
since $\alpha$ is simple.
Therefore, $b_1^1\ne 0$.

Similarly, $B(e_1)\w(e_{1}\w e_{3}\w \ldots  \w e_d) = -b^2_1\Omega$. 
So, if $b^2_1 = 0$, then $e_1(\rho(\beta\alpha\beta^{-1}))$,
lies in the hyperplane spanned by
$\{e_1(\rho(\alpha)),e_3(\rho(\alpha)),\ldots,e_d(\rho(\alpha))\}$,
which again contradicts Corollary \ref{productnonzero}.
Therefore, $b^2_1 \neq 0$.

Moreover,
$B(e_2)\w(e_2\w e_{3}\w \ldots  \w e_d) = b^1_2 \Omega$. 
So, if $b^1_2 = 0$, then $e_2(\rho(\beta\alpha\beta^{-1}))$,
lies in the hyperplane spanned by
$\{e_1(\rho(\alpha)),e_3(\rho(\alpha),\ldots,e_d(\rho(\alpha)\}$,
which again contradicts Corollary \ref{productnonzero}.
Thus, $b^1_2\neq 0$.
\end{proof}


By assumption $|\lambda_1(A^nB)| = |\lambda_1(\hat A^n\hat B)|$ for all $n$. 
Lemma \ref{specradiusexpansion} then implies that
$$\left| b^1_1 + \frac{b^1_2b^2_1}{b^1_1} \left(\frac{\lambda_2}{\lambda_1}\right)^n+ o\left(\left(\frac{\lambda_2}{\lambda_1}\right)^n\right) \right|= \left|\hat b^1_1 + \frac{\hat b^1_2\hat b^2_1}{\hat b^1_1} \left(\frac{\hat\lambda_2}{\hat\lambda_1}\right)^n+o\left(\left(\frac{\hat\lambda_2}{\hat\lambda_1}\right)^n\right)\right|,$$
so
$|b^1_1| = |\hat b^1_1|.$
Comparing  the second order terms, we see that
$$\frac{\lambda_2}{\lambda_1}= \frac{\hat\lambda_2}{\hat\lambda_1}.$$
Since, by assumption, $\lambda_1=\hat\lambda_1$, we see that $\lambda_2=\hat\lambda_2$.


We now assume  that for some $k=2,\ldots, d-1$,
$\lambda_i(\rho(\beta))=\lambda_i(\sigma(\beta))$ for all $i\le k$ whenever $\beta\in\braket{\gamma,\delta}$ is represented
by a simple, non-separating based loop.
We will prove that this implies that 
$\lambda_i(\rho(\alpha))=\lambda_i(\sigma(\alpha))$ for all $i\le k+1$ whenever $\alpha\in\braket{\gamma,\delta}$ is represented
by a simple, non-separating based loop.
Applying this iteratively  will allow us to complete the proof.


Let $E^{k}(\rho)$ be the $k^{th}$-exterior product representation. 
If $\alpha\in\braket{\gamma,\delta}$ is represented by a simple non-separating based loop, we again choose
$\beta\in\braket{\gamma,\delta}$  so that $\beta$ is represented by a simple based loop which intersects
$\alpha$ only at the basepoint and $\alpha$ and $\beta$ have geometric intersection one. We adapt the notations
and conventions from the second paragraph of the proof.

Let $C= E^{k}(\rho)(\alpha)$, $D=E^k(\rho)(\beta)$, $\hat C=E^k(\sigma)(\alpha)$ and
$\hat D=E^k(\sigma)(\beta)$. Notice that $C$ and $C^nD$ are real-split and 2-proximal for all $n$.
If $c_i=e_i(C)$, then we may assume that each $c_i$ is a $k$-fold wedge product of
distinct $e_j$. In particular, we may take $c_1=e_1\w e_2\w \ldots \w e_k$ and
$c_2=e_1\w e_2\w \ldots \w e_{k-1}\w e_{k+1}$. Notice that  
$\lambda_1(C)=\lambda_1\cdots\lambda_k$ and $\lambda_2(C)=\lambda_1\cdots\lambda_{k-1}\lambda_{k+1}$.
Let $(d^i_j)$ be the matrix for $D$ in the basis $\{c_i\}$. We define $\hat c_i$ and $(\hat d^i_j)$ completely
analogously.

Notice that $D(e_1\w e_2\w \ldots \w e_k)\w (e_{k+1}\w \ldots  \w e_d) = d^1_1\Omega$. So, if $d^1_1=0$, then 
$$B(\xi_\rho^k(\alpha_+))\oplus\xi_\rho^{n-k}(\alpha_-)  = \xi_\rho^k(\beta(\alpha_+)) \oplus \xi_\rho^{n-k}(\alpha_-) \neq \Real^d.
$$
which would contradict the hyperconvexity of $\xi_\rho$. Therefore, $d_1^1\ne 0$.
 
Furthermore, $D(e_1\w e_2\w \ldots \w e_k)\w(e_{k}\w e_{k+2}\w \ldots  \w e_d) = -d^2_1\Omega$. 
So, if $d^2_1 = 0$, then
$$\left\{L_1(\rho(\beta\alpha\beta^{-1})),\ldots,L_k(\rho(\beta\alpha\beta^{-1})),L_k(\rho(\alpha)),L_{k+2}(\rho(\alpha)),\ldots,
L_d(\rho(\alpha))\right\}$$
does not span $\mathbb R^d$, which contradicts Corollary \ref{productnonzero}.
Therefore, $d^2_1 \neq 0$

Similarly, $D(e_1\w e_2\w \ldots \w e_{k-1} \w e_{k+1})\w(e_{k+1}\w e_{k+2}\w \ldots  \w e_d) = d^1_2 \Omega$. 
So, if $d^1_2 = 0$, then
$$\left\{L_1(\rho(\beta\alpha\beta^{-1})),\ldots,L_{k-1}(\rho(\beta\alpha\beta^{-1})),L_{k+1}(\rho(\beta\alpha\beta^{-1})),L_{k+1}(\rho(\alpha)),\ldots,
L_d(\rho(\alpha))\right\}$$
does not span $\mathbb R^d$, which contradicts Corollary \ref{productnonzero}.
Thus $d^1_2\neq 0$.

Analogous arguments imply that $\hat d^1_1$, $\hat d_1^2$ and $\hat d_2^1$ are all non-zero. Moreover,
by our iterative assumption
$$|\lambda_1(C^nD)|=|\lambda_1(A^nB)\cdots\lambda_k(A^nB)|=
|\lambda_1(\hat A^n\hat B)\cdots\lambda_k(\hat A^n\hat B)|=| \lambda_1(\hat C^n\hat D)|$$
for all $n$. We may
again apply Lemma \ref{specradiusexpansion} to conclude that
$$\frac{\lambda_{k+1}}{\lambda_k} = \left|\frac{\lambda_2(C)}{\lambda_1(C)}\right|= \left| \frac{\lambda_2(\hat C)}{\lambda_1(\hat C)}\right|= 
\frac{\hat\lambda_{k+1}}{\hat\lambda_k}.$$
Since, by our inductive assumption, $\lambda_k=\hat\lambda_k$, we conclude that
$\lambda_{k+1}=\hat\lambda_{k+1}$.\
Therefore, after iteratively applying our argument, we conclude that 
$\lambda_i(\rho(\alpha))=\hat\lambda_i(\sigma(\alpha))$ for all $i$,
so $|\tr(\rho(\alpha))|=|\tr(\sigma(\alpha))|$.
\end{proof}



==> proj_lengthtrace-resubmit.tex <==

%% !TEX root =HitchinSimple.tex
\subsection{Projective Lengths}
We now prove a projective version of Lemma \ref{length to trace}.
\begin{lemma}
\label{proj_length to trace}
If $\rho,\sigma \in  {\mathcal H}_d(S)$ and there exists  a $r > 0$ such that
$L_{\alpha}(\rho)=r.L_{\alpha}(\sigma)$ whenever $\alpha$ is represented by
a simple non-separating based loop, then $r=1$,
$|\tr(\rho(\alpha))|=|\tr(\sigma(\alpha))|$ and
$\lambda_i(\rho(\alpha))=\lambda_i(\sigma(\alpha))$ for all $i$ 
where $\alpha$ is represented by
a simple non-separating based loop.
\end{lemma}

\begin{proof} 
We will show that $r = 1$ and then the result follows from above. We will use the same notaton as in Lemma \ref{length to trace}.  By Lemma \ref{specradiusexpansion}  implies that there are analytic functions $f, \hat f$ such that 
$$\frac{\lambda_1(A^nB)}{\lambda_1(A^n)} = f\left(\left(\frac{\lambda_2}{\lambda_1}\right)^n,\ldots, \left(\frac{\lambda_d}{\lambda_1}\right)^n\right)  = b^1_1 + \sum_{k=1}^d\frac{b^1_kb^k_1}{b^1_1} \left(\frac{\lambda_k}{\lambda_1}\right)^n+ o\left(\left(\frac{\lambda_2}{\lambda_1}\right)^n\right) $$
$$\frac{\lambda_1(\hat A^n\hat B)}{\lambda_1(\hat A^n)} = \hat f \left(\left(\frac{\hat\lambda_2}{\hat\lambda_1}\right)^n,\ldots, \left(\frac{\hat\lambda_d}{\hat\lambda_1}\right)^n\right)  = \hat b^1_1 + \sum_{k=2}^d\frac{\hat b^1_k\hat b^k_1}{\hat b^1_1} \left(\frac{\hat\lambda_k}{\hat\lambda_1}\right)^n+o\left(\left(\frac{\hat\lambda_2}{\hat\lambda_1}\right)^n\right).$$
By assumption $|\lambda_1(A^nB)| = |\lambda_1(\hat A^n\hat B)|^r$ for all $n$.  Therefore
$$\left|f\left(\left(\frac{\lambda_2}{\lambda_1}\right)^n,\ldots, \left(\frac{\lambda_d}{\lambda_1}\right)^n\right) \right|=  \left|\hat f\left(\left(\frac{\hat\lambda_2}{\hat\lambda_1}\right)^n,\ldots, \left(\frac{\hat\lambda_d}{\hat\lambda_1}\right)^n\right)\right|^r$$
Therefore taking a limit as $n$ goes to infinity, we get  $|f(0)| =|\hat f(0)|^r$ giving $|b^1_1| = |\hat b^1_1|^r.$
Taking logs we obtain analytic functions $g, \hat g $ such that

$$ g =  \log\left| 1 + \sum_{k=2}^d\frac{b^1_kb^k_1}{(b^1_1)^2} \left(\frac{\lambda_k}{\lambda_1}\right)^n+ o\left(\left(\frac{\lambda_2}{\lambda_1}\right)^n\right) \right| = r\log\left| 1+ \sum_{k=2}^d\frac{\hat b^1_k\hat b^k_1}{(\hat b^1_1)^2} \left(\frac{\hat\lambda_k}{\hat\lambda_1}\right)^n+o\left(\left(\frac{\hat\lambda_2}{\hat\lambda_1}\right)^n\right)\right| =\hat g$$
 Comparing  the highest order term, we have that
$$\frac{\lambda_2}{\lambda_1}= \frac{\hat\lambda_2}{\hat\lambda_1}.$$

{\bf Problem here:}  I was thinking we could now eliminate all terms with $\lambda_2/\lambda_1$ and move to next highest term not involving $\lambda_2/\lambda_1$ which would imply $\lambda_3/\lambda_1$ are equal. Repeating you'd then get all $\lambda_k/\lambda_1$ are equal and together with $\lambda_1 = \hat\lambda_1^r$ you have $r =1$.

The issue is there could be resonances like $(\lambda_2/\lambda_1)^2 = \lambda_3/\lambda_1$. One possibility is that we only need a single  $\alpha$ without resonances to derive $r=1$. Could be ugly, might need to argue case by case for the Zariski closures.
\end{proof}


